A lattice on Dyck paths close to the Tamari lattice

We introduce a new poset structure on Dyck paths where the covering relation is a particular case of the relation inducing the Tamari lattice. We prove that the transitive closure of this relation endows Dyck paths with a lattice structure. We provide a trivariate generating function counting the number of Dyck paths with respect to the semilength, the numbers of outgoing and incoming edges in the Hasse diagram. We deduce the numbers of coverings, meet and join irreducible elements. As a byproduct, we present a new involution on Dyck paths that transports the bistatistic of the numbers of outgoing and incoming edges into its reverse. Finally, we give a generating function for the number of intervals, and we compare this number with the number of intervals in the Tamari lattice.

==> antoine_package.tex <==
\usepackage{booktabs}
\usepackage{etex}
\usepackage{multirow}
%\setcounter{tocdepth}{3}
%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm}
\usepackage{amsfonts}

\usepackage{pdfpages}
\usepackage{url}
\usepackage{hyperref}
\usepackage{enumerate}
\usepackage{tikz}
\usetikzlibrary{decorations.markings, calc,automata}
\usepackage{stmaryrd}
\usepackage{color}
%\usepackage[dvipsnames]{xcolor}

%\usepackage{wrapfig}
%\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{tikz}
\usepackage{stmaryrd}
\usepackage{color}
\usepackage{pdfpages}


\usepackage[]{algorithm}
\usepackage{etoolbox}\AtBeginEnvironment{algorithmic}{\footnotesize} 
\usepackage[noend]{algpseudocode}
\usepackage{mathrsfs}
\usepackage{caption}


\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}

\newcommand{\I}{\mathcal{I}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
%\renewcommand{\O}{\mathcal{O}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\R}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\Q}{\mathcal{Q}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}


\newcommand{\IE}{\mathbb{E}}
\newcommand{\IV}{\mathbb{V}}
\newcommand{\IC}{\mathbb{C}}
\newcommand{\IN}{\mathbb{N}}
\newcommand{\IP}{\mathbb{P}}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\BigO}{\mathcal{O}}

\DeclareRobustCommand{\stirling}{\genfrac\{\}{0pt}{}}


\newcommand{\Bern}{\mbox{Bern}}
\newcommand{\Geom}{\mbox{Geom}}
\newcommand{\Seq}{\mbox{\sc Seq}}
\newcommand{\SeqUn}{\mbox{\sc Seq}_{\geq 1}}
\newcommand{\SeqDeux}{\mbox{\sc Seq}_{\geq 2}}
\newcommand{\SeqTrois}{\mbox{\sc Seq}_{\geq 3}}
\newcommand{\SeqQ}{\mbox{\sc Seq}_{\geq 4}}
\newcommand{\Seqk}{\mbox{\sc Seq}_{\geq k}}
\newcommand{\Seql}{\mbox{\sc Seq}_{\geq \ell}}
\newcommand{\Set}{\mbox{\sc Set}}
\newcommand{\SetUn}{\mbox{\sc Set}_{\geq 1}}
\newcommand{\MSet}{\mbox{\sc MSet}}
\newcommand{\PSet}{\mbox{\sc PSet}}
\newcommand{\Cycle}{\mbox{\sc Cyc}}
\newcommand{\Shuf}{\mbox{\sc Shuf}}
\newcommand{\LSeq}{\mbox{\sc Lseq}}
\newcommand{\Tree}{\mbox{\sc Tree}}

%\newcommand{\bs}{\boldsymbol}
%\newcommand{\cec}{\color{magenta}}
%\newcommand{\meh}{\color{teal}}
% 	\definecolor{forestgreen(traditional)}{rgb}{0.0, 0.27, 0.13}

\newcommand{\bs}{\boldsymbol}
\newcommand{\sss}{\scriptscriptstyle}


%{\theoremstyle {plain} \newtheorem{theorem}{Theorem}[subsection]}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}
%\newtheorem{properties}[theorem]{Properties}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
%\newtheorem{remark}[theorem]{Remark}

%\theoremstyle{definition}
\newtheorem{Definition}[theorem]{Definition}
\newtheorem{Definitions}[theorem]{Definitions}


\tikzset{
node distance=2cm, % specifies the minimum distance between two nodes. Change if necessary.
every state/.style={ fill=gray!10}, % sets the properties for each ’state’ node
initial text=$ $ % sets the text that appears on the start arrow
}


%\newcommand{\qed}{\ensuremath{\hfill \square}}

%\newproof{@proof}{Proof} 
%\newenvironment{proof}{\begin{@proof}}{\qed \end{@proof}} 


%%---a supprimer
\newcommand{\nnote}[2][]{\textcolor{red}{\textsc{Note #1:} \emph{#2}}}
%\newcommand{\MP}[1]{\marginpar{\textcolor{red}{\footnotesize #1}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> sections/conclusion.tex <==

\section{Conclusion}\label{sec:conclu}

\section{J.-L.'s delusions}

Let $\mathcal{D}_n$ be the set of Dyck paths of semi-length $n$ and $\mathcal{D}=\cup_{n\geq 0} \mathcal{D}_n$.
Let $P$ be a Dyck path in $\mathcal{D}_n$. Below, we define the Stanley-code (already known) and the BKN-shape of $P$.

\noindent {\bf Stanley code:} Let $c(P)=c_1c_2\ldots c_n$ be the length $n$ Stanley-code of $P$, i.e. $c_i$ is the number of up-steps before the $i$-th down-step. For instance, if $P=UUUDUUDDDUUDDD$ then $c(P)=3555777$.

Clearly, a Stanley code $c_1c_2\ldots c_n$ of a Dyck path satisfies:

\begin{enumerate}
    \item[($i$)] $i\leq c_i\leq n$ for $1\leq i\leq n$,
    \item[($ii$] $c_i\leq c_{i+1}$ for $1\leq i\leq n-1$.
\end{enumerate}


Conversely, if $c=c_1c_2\ldots c_n$ satisfies ($i$) and ($ii$), then $c$ is the Stanley code of a Dyck path of semi-length $n$.

\begin{remark} The poset defined on the Stanley codes of length $n$  by the relation $c_1c_2\ldots c_n\leq d_1d_2\ldots d_n$, is a ranked distributive lattice (already known) 
\end{remark}


\noindent {\bf BKN-shape:} Let $s(P)=\{s_1,s_2,\ldots, s_k\}$, $k\leq n$, be the length $n$ BKN-shape of $P$, i.e. $s_i$ is the number of up-steps before the $i$-th peak, knowing that a peak is a point of the path between an up-step $U$ and a down-step $D$ ($U$ and $D$ being consecutive). For instance, if $P=UUUDUUDDDUUDDD$ then $c(P)=\{s_1,s_2,s_3\}=\{3,5,7\}$ (and thus $k=3$ in this case).

\begin{remark} The BKN-shape of a Dyck path $P$, is the set of values in the Stanley-code $c(P)$.
\end{remark}

\begin{remark}  Two different Dyck paths can have the same BKN-shape. For instance, $P=UUDUDD$ and $Q=UUDDUD$ have the same BKN-shape $s(P)=s(Q)=\{2,3\}$.
\end{remark}



\noindent{\bf TO check! Maybe wrong!}

\begin{theorem} Let $\rightarrow$ be the Tamari-rotation on Dyck paths and $\stackrel{*}{\rightarrow}$ the reflexive transitive closure of $\rightarrow$.

 Let $P$ and $Q$ be two Dyck paths of the same semi-length. Then we have $$P\stackrel{*}{\rightarrow} Q \quad \Longleftrightarrow 
 \left\{\begin{array}{l}
 c(P)\leq c(Q)\\
 s(Q)\subseteq s(P)\end{array}\right.$$
\end{theorem}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper_discrete.tex"
%%% End:


==> sections/general_setting.tex <==
\section{The transformation}



==> sections/intro.tex <==
\section{Introduction}\label{sec:intro}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper_discrete.tex"
%%% End:

